Unbiased Teacher for Semi-Supervised Object Detection

Semi-supervised learning, i.e., training networks with both labeled and unlabeled data, has made significant progress recently. However, existing works have primarily focused on image classification tasks and neglected object detection which requires more annotation effort. In this work, we revisit the Semi-Supervised Object Detection (SS-OD) and identify the pseudo-labeling bias issue in SS-OD. To address this, we introduce Unbiased Teacher, a simple yet effective approach that jointly trains a student and a gradually progressing teacher in a mutually-beneficial manner. Together with a class-balance loss to downweight overly confident pseudo-labels, Unbiased Teacher consistently improved state-of-the-art methods by significant margins on COCO-standard, COCO-additional, and VOC datasets. Specifically, Unbiased Teacher achieves 6.8 absolute mAP improvements against state-of-the-art method when using 1% of labeled data on MS-COCO, achieves around 10 mAP improvements against the supervised baseline when using only 0.5, 1, 2% of labeled data on MS-COCO.

==> figures/ablation-fixmatch.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/pic/ablation-fixmatch.pdf}
%     \caption{Experimental result on our proposed model and the method based on FixMatch~\cite{sohn2020fixmatch}. It demonstrated that the using MMA-based updating mechanism can help the object detection learning in the semi-supervised setting. }
%     \label{fig:overview_model}
% \end{figure}

\begin{figure*}[t]
   \begin{picture}(0,150)
     \put(0,15){\includegraphics[width=7.5cm]{figures/pic/ablation-fixmatch.pdf}}
     \put(200,15){\includegraphics[width=7.5cm]{figures/pic/ablation-fixmatch-tide.pdf}}
    % \put(200,15){\includegraphics[width=7.5cm]{figures/pic/ablation-emaonoff-apbreakdown.pdf}}

     \put(105,5){(a)}
     \put(305,5){(b)}

   \end{picture}
\vspace{-5mm}
    \caption{(a) Our model with EMA training can perform favorably against our model without EMA training. (b) using EMA training leads to significant lower Miss error (\textit{i.e.,} higher recall) but slightly degrade the performance of foreground predictions (\textit{i.e.,} lower precision; Higher Cls, Loc, Both, Duplicate, Bkg errors). }
\label{fig:ablation-mma_training}
\end{figure*}


==> figures/ablation-loss-apendix.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/pic/ablation-loss.pdf}
%     \caption{Performance gap between Focal loss and cross-entropy.}
%     \label{fig:overview_model}
% \end{figure}
\begin{figure*}[t]
   \begin{picture}(0,150)
     \put(0,15){\includegraphics[width=7.5cm]{figures/pic/ablation-loss.pdf}}
     \put(200,15){\includegraphics[width=7.5cm]{figures/pic/ablation-loss-apbreakdown.pdf}}

     \put(97,8){(a)}
     \put(297,8){(b)}

   \end{picture}
\vspace{-5mm}
    \caption{Performance gap between Focal loss and cross-entropy.\yencheng{ Pseudo-labels histogram is better?} }
\label{fig:ablation-loss-appendix}
\end{figure*}



==> figures/ablation-loss.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/pic/ablation-loss.pdf}
%     \caption{Performance gap between Focal loss and cross-entropy.}
%     \label{fig:overview_model}
% \end{figure}
\begin{figure*}[t]
   \begin{picture}(0,150)
     \put(0,15){\includegraphics[width=7.5cm]{figures/pic/ablation-loss.pdf}}
    %  \put(200,15){\includegraphics[width=7.5cm]{figures/pic/ablation-loss-apbreakdown.pdf}}

     \put(97,8){(a)}
     \put(297,8){(b)}

   \end{picture}
\vspace{-5mm}
    \caption{Performance gap between Focal loss and cross-entropy.\yencheng{ Pseudo-labels histogram is better?} }
\label{fig:ablation-loss}
\end{figure*}



==> tables/ablation-backbone.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{\textcolor{blue}{ Experimental results on ResNeXt101-FPN on \textit{COCO-standard} 1\% labeled data setting.}
    }
    \vspace{2mm}
\label{table:mscoco-additional}
\resizebox{0.3\linewidth}{!}{%
\begin{tabular}{ccc}
\toprule
          & \multicolumn{2}{c}{COCO-standard 1\%}  \\ \cline{2-3}
          & Supervised & Ours \\ \hline
$AP^{50:95}$& 13.87 & 24.58    \\ 
\bottomrule
\end{tabular}}
\vspace{-5mm}
\end{table}


==> tables/ablation-ema_rate.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
Ablation study of varying MMA rate $\alpha$ on the model trained using $1\%$ labeled and $99\%$ unlabeled data.}
\label{table:ablation_mma_rate}
\begin{tabular}{lccccccc}
\toprule
MMA rate ($\alpha$)   & 0        &  0.5      &  0.9   & 0.99  & 0.999 & 0.9996 & 0.9999\\ \hline
AP ($\%$)             &   17.41  &    17.81  & 17.07  & 21.1    &  21.06 & 21.19 & 20.13      \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation-thres.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
Ablation study of varying pseudo-labeling threshold $\delta$ on the model trained using $1\%$ labeled and $99\%$ unlabeled data.}
\label{table:ablation_thres}
\begin{tabular}{lcccccc}
\toprule
$\delta$   & 0                   &  0.5            &  0.6  & 0.7    &  0.8    & 0.9\\ \hline
AP ($\%$)  &   Cannot converge  & Cannot converge  & 17.80 & 21.19  &  13.58 & 9.88 \\ 
\bottomrule
\end{tabular}
\end{table}

==> tables/ablation.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3}
% \caption{
%     Ablation study on MS-COCO~\citep{lin2014microsoft} using 1\% labeled data. 
%     }
% \begin{tabular}{lllll}
% \Xhline{2\arrayrulewidth}
% & \multicolumn{4}{l}{1\% Labeled data on MS-COCO} \\ \cline{2-5} 
% & \begin{tabular}[c]{@{}l@{}}Supervised\\ pre-training\end{tabular} & EMA & \begin{tabular}[c]{@{}l@{}}Focal\\ loss\end{tabular} & AP \\ \hline
% Supervised & & & &    \\
% \multirow{5}{*}{} & & & &    \\
% & & & &    \\
% & & & &    \\
% & & & &    \\
% & & & & \\
% \Xhline{2\arrayrulewidth}
% \end{tabular}
% \end{table}

% ================================================

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\caption{
    Ablation study on MS-COCO~\citep{lin2014microsoft} using 1\% labeled data. 
    }
\label{table:ablation}
\begin{tabular}{cccccc}
\Xhline{2\arrayrulewidth}
& \multicolumn{5}{c}{1\% Labeled data on MS-COCO} \\ \cline{2-6} 
& \# & Supervised Pre-training & EMA & Focal Loss & AP \\ \hline
Supervised & & & &    \\ \hline
\multirow{5}{*}{\ProposedMethodName} & 1 & & &    \\
& 2 & & & &    \\
& 3 & & & &    \\
& 4 & & & &    \\
& 5 & \checkmark & \checkmark & \checkmark & \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\end{table}
